The effect of stellar rotation on black hole mass and spin

The gravitational wave signature of a binary black hole (BBH) merger is dependent on its component mass and spin. If such black holes originate from rapidly rotating progenitors, the large angular momentum reserve in the star could drive a collapsar-like supernova explosion, hence substantially impacting these characteristics of the black holes in the binary. To examine the effect of stellar rotation on the resulting black hole mass and spin, we conduct a 1D general relativistic study of the end phase of the collapse. We find that the resulting black hole mass at times differs significantly from the previously assumed values. We quantify the dependence of the black hole spin magnitude on the hydrodynamics of the accretion flow, providing analytical relations for calculating the mass and spin based on the progenitor's pre-collapse properties. Depending on the nature of the accretion flow, our findings have implications for the black hole upper mass gap resulting from pair-instability supernovae, the maximum mass of a maximally rotating stellar black hole, and the maximum effective spin of a BBH formed in tidally locked helium star - black hole binary.

==> table2.tex <==
\begin{table}
% \vspace{-10pt}
    \centering
    \caption{For convenience, here we redefine some key variables used in this work.}
    \label{tab: variables}
    
    \begin{tabular}{cc} % four columns, alignment for each
    \hline
    
     Variable  &  Significance \\
    \hline \hline
    $M$ or $M_{\rm BH}$  & Mass of the black hole. \\ 
    $a$ & Kerr spin parameter of the black hole. \\
    $a^*:= a/M$  & Dimensionless spin parameter of the black hole. \\
    $\dot{M}_{\rm BH}$ & Rate of mass accretion by the black hole \\
    $\dot{J}_{\rm BH}$ & Rate of angular momentum accretion by the black hole. \\
    $\dot{M}_d$ & Rate of change of mass of the disk. \\
    $\dot{M}_{\rm wind}$ & Rate of loss of mass in disk winds. \\
    $\dot{J}_{\rm wind}$ & Rate of loss of angular momentum in disk winds. \\
    $r_t$ & Transitional radius below which no wind mass loss occurs. \\
    $r_d$ & Characteristic disk radius. \\
    $\ell(r)$ & In plane specific angular momentum at radius $r$. \\
    \hline
    \end{tabular}
\end{table}

